Design of a Health Monitoring System for a Planetary Exploration Rover

It is generally considered that a trustworthy autonomous planetary exploration rover must be able to operate safely and effectively within its environment. Central to trustworthy operation is the ability for the rover to recognise and diagnose abnormal behaviours during its operation. Failure to diagnose faulty behaviour could lead to degraded performance or an unplanned halt in operation. This work investigates a health monitoring method that can be used to improve the capabilities of a fault detection system for a planetary exploration rover. A suite of four metrics, named 'rover vitals', are evaluated as indicators of degradation in the rover's performance. These vitals are combined to give an overall estimate of the rover's 'health'. By comparing the behaviour of a faulty real system with a non-faulty observer, residuals are generated in terms of two high-level metrics: heading and velocity. Adaptive thresholds are applied to the residuals to enable the detection of faulty behaviour, where the adaptive thresholds are informed by the rover's perceived health. Simulation experiments carried out in MATLAB showed that the proposed health monitoring and fault detection methodology can detect high-risk faults in both the sensors and actuators of the rover.

==> sections/testCaseBfig.tex <==
\begin{figure*}[tbp]
    \begin{subfigure}[t]{0.32\textwidth}
        \includegraphics[width=\linewidth]{figs/2024_02_08_rover_health_heading_abrupt_10_deg_reformatting.eps}
        \caption{Test case A: rover health in the presence of no faults} \label{fig:a}
    \end{subfigure}\hspace*{\fill}
    \begin{subfigure}[t]{0.32\textwidth}
        \includegraphics[width=\linewidth]{figs/2024_01_04_heading_residual_no_fault.eps}
        \caption{Test case A: Heading residual with adaptive threshold in the presence of no faults} \label{fig:b}
    \end{subfigure} \hspace*{\fill}
    \begin{subfigure}[t]{0.32\textwidth}
        \includegraphics[width=\linewidth]{figs/2024_01_04_velocity_residual_no_fault.eps}
        \caption{Test case A: Velocity residual with adaptive threshold in the presence of no faults} \label{fig:c}     
    \end{subfigure} 
   
    \caption{Health Monitoring and Adaptive Threshold Generation for Test Cases A, B, and C} \label{fig:healthAndAdaptiveThresholds}
    
\end{figure*}

==> sections/testCaseCFig.tex <==
\begin{figure*}[tbp]
    \begin{subfigure}[t]{0.32\textwidth}
        \includegraphics[width=\linewidth]{figs/2024_01_04_rover_health_dead_motor.eps}
        \caption{Test case A: rover health in the presence of no faults} \label{fig:a}
    \end{subfigure}\hspace*{\fill}
    \begin{subfigure}[t]{0.32\textwidth}
        \includegraphics[width=\linewidth]{figs/2024_01_04_heading_residual_no_fault.eps}
        \caption{Test case A: Heading residual with adaptive threshold in the presence of no faults} \label{fig:b}
    \end{subfigure} \hspace*{\fill}
    \begin{subfigure}[t]{0.32\textwidth}
        \includegraphics[width=\linewidth]{figs/2024_01_04_velocity_residual_no_fault.eps}
        \caption{Test case A: Velocity residual with adaptive threshold in the presence of no faults} \label{fig:c}     
    \end{subfigure} 
   
    \caption{Health Monitoring and Adaptive Threshold Generation for Test Cases A, B, and C} \label{fig:healthAndAdaptiveThresholds}
    
\end{figure*}
